Scene-Generalizable Interactive Segmentation of Radiance Fields

Existing methods for interactive segmentation in radiance fields entail scene-specific optimization and thus cannot generalize across different scenes, which greatly limits their applicability. In this work we make the first attempt at Scene-Generalizable Interactive Segmentation in Radiance Fields (SGISRF) and propose a novel SGISRF method, which can perform 3D object segmentation for novel (unseen) scenes represented by radiance fields, guided by only a few interactive user clicks in a given set of multi-view 2D images. In particular, the proposed SGISRF focuses on addressing three crucial challenges with three specially designed techniques. First, we devise the Cross-Dimension Guidance Propagation to encode the scarce 2D user clicks into informative 3D guidance representations. Second, the Uncertainty-Eliminated 3D Segmentation module is designed to achieve efficient yet effective 3D segmentation. Third, Concealment-Revealed Supervised Learning scheme is proposed to reveal and correct the concealed 3D segmentation errors resulted from the supervision in 2D space with only 2D mask annotations. Extensive experiments on two real-world challenging benchmarks covering diverse scenes demonstrate 1) effectiveness and scene-generalizability of the proposed method, 2) favorable performance compared to classical method requiring scene-specific optimization.

==> figures/fig_additional_ablation.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=0.90\linewidth]{figures/ablation/ablation_additional_v2.pdf}
\vspace{-8pt}
\caption{Visualization of rendering segmented foreground scenes. `U', `P', `O1', `O'and `O' denote `Uncertainty-Eliminated 3D segmentation’, `Cross-Dimension Guidance Propagation', ‘Object-Exclusive Segmentation Supervision with only $\mathcal{L}_\text{obj}^1$’ , ‘Object-Exclusive Segmentation Supervision with only $\mathcal{L}_\text{obj}^2$’ and `the total Object-Exclusive Segmentation Supervision’ respectively.}
\label{fig:addition ablation1}
% \vspace{-8pt}
\end{figure*}

==> figures/fig_additional_ablation_llff.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=0.82\linewidth]{figures/appendix/additional_ablation_llff_v2.pdf}
\vspace{-10pt}
\caption{Additional Visual Ablation corresponding to Figure 6 in paper.  Visualization of rendering segmented foreground scenes. `U', `P' and `O' denote `Uncertainty-Eliminated 3D segmentation’, `Cross-Dimension Guidance Propagation' and `Object-Exclusive Segmentation Supervision’ respectively.
While `Cross-Dimension Guidance Propagation' enables our model to segment more accurate foreground, `Object-Exclusive Segmentation Supervision’ can reveal and correct the false positive predictions as highlighted by red dashed boxes.}
\label{fig:appedix-ablation}
% \vspace{-10pt}
\end{figure*}

==> figures/fig_additional_co3d.tex <==
% set for \usepackage{stfloats}
% \begin{figure*}[hb] 
\begin{figure*}[!t]
\centering
\includegraphics[width=0.82\linewidth]{figures/appendix/co3d_additionanl_comparision.pdf}
\vspace{-10pt}
\caption{Qualitative comparison with NVOS on CO3D dataset. Our method outperforms NVOS on both cases.  As highlighted by red dashed boxes, our method even produces more precise segmentation than the groundtruth.}
\label{fig:appedix-co3d}
%\vspace{2pt}
\end{figure*}

==> figures/fig_additional_llff.tex <==
% set for \usepackage{stfloats}
% \begin{figure*}[hb] 
\begin{figure*}[!t]
\centering
\includegraphics[width=0.82\linewidth]{figures/appendix/llff_additional_result_v5.pdf}
\vspace{-10pt}
\caption{Visual Comparison with NVOS on NeRF-LLFF. The positive and negative user interactions are indicated by blue and red points, respectively. As highlighted by red dashed boxes, our method segments the rib-cage bones of T-Rex more finely.}
\label{fig:appedix-comparsion-llff}
% \vspace{-10pt}
\end{figure*}
